3-D CMZ II: Hierarchical Structure Analysis of the Central Molecular Zone

The Central Molecular Zone (CMZ) is the way station at the heart of our Milky Way Galaxy, connecting gas flowing in from Galactic scales with the central nucleus. Key open questions remain about its 3-D structure, star formation properties, and role in regulating this gas inflow. In this work, we identify a hierarchy of discrete structures in the CMZ using column density maps from Paper I (Battersby et al., submitted). We calculate the physical ($N$(H$_2$), $T_{\rm{dust}}$, mass, radius) and kinematic (HNCO, HCN, and HC$_3$N moments) properties of each structure as well as their bolometric luminosities and star formation rates (SFRs). We compare these properties with regions in the Milky Way disk and external galaxies. Despite the fact that the CMZ overall is well below the Gao-Solomon dense gas star-formation relation (and in modest agreement with the Schmidt-Kennicutt relation), individual structures on the scale of molecular clouds generally follow these star-formation relations and agree well with other Milky Way and extragalactic regions. We find that individual CMZ structures require a large external pressure ($P_e$/k$_B$ $> 10^{7-9}$ K cm$^{-3}$) to be considered bound, however simple estimates suggest that most CMZ molecular-cloud-sized structures are consistent with being in pressure-bounded virial equilibriuim. We perform power-law fits to the column density probability distribution functions (N-PDFs) of the inner 100 pc, SgrB2, and the outer 100 pc of the CMZ as well as several individual molecular cloud structures and find generally steeper power-law slopes ($-9<\alpha<-2$) compared with the literature ($-6 < \alpha < -1$).

==> final_sfr_v2.tex <==
\begin{table*}
\centering
\caption{Luminosity properties of the dendrogram structures. Shown for each structure is the source name, structure ID, total luminosity and mean luminosity for the cool and warm components, respectively, the combined total IR luminosity, the SFR inferred from that total IR luminosity assuming the star-forming relation from \citet{Kennicutt1998}, the SFR estimated using the method from \citet{Barnes2017} but using the free-fall time, the SFR reported in matching sources from the CMZoom catalog \citep{Hatchfield2024} and the corresponding uncertainty, and the best overall SFR estimate for each structure. The grouping and order of structures is the same as in Table \ref{tab:general_properties}. $^{*}$See section \ref{sec:sfr} for details regarding the choice of best SFR estimate. No best SFR estimate is given for branches with A \textless\ 1000~pc$^{-2}$.}\resizebox{\linewidth}{!}{%
\begin{tabular}{cccccccccccccc}
\hline
Name & ID & L$_{\textrm{tot}}$ & $\langle L \rangle$ & L$_{\textrm{tot}}$ & $\langle L \rangle$ & L$_{\textrm{total IR}}$ & SFR$_{\textrm{total IR}}$ & SFR$_{\textrm{FF}}$ & SFR$_{\textrm{CMZoom}}$ & ERR$_{\textrm{CMZoom}}$ & SFR$_{\textrm{CMZoom}}$ & ERR$_{\textrm{CMZoom}}$ & \textbf{Best SFR} \\
& & (Cool) & (Cool) & (Warm) & (Warm) & & & & Herschel temp & Herschel temp & 50K & 50K  &\textbf{Estimate$^{*}$} \\ \hline
& & $\mathrm{L_{\odot}}$ & $\mathrm{L_{\odot}}$/pix & $\mathrm{L_{\odot}}$ & $\mathrm{L_{\odot}}$/pix & $\mathrm{L_{\odot}}$ & $\mathrm{M_{\odot}\,yr^{-1}}$ & $\mathrm{M_{\odot}\,yr^{-1}}$ & $\mathrm{M_{\odot}\,yr^{-1}}$  & $\mathrm{M_{\odot}\,yr^{-1}}$ & $\mathrm{M_{\odot}\,yr^{-1}}$ & $\mathrm{M_{\odot}\,yr^{-1}}$ &$\mathrm{M_{\odot}\,yr^{-1}}$ \\ \hline
Branches & \\ \hline
G0.720-0.069 & 8 & 1.4E+08 & 2.2E+03 & 6.1E+07 & 1.7E+03 & 2.1E+08 & 3.5E-02 & - & - & - & - & - & 3.5E-02 \\
G0.750-0.070 & 9 & 1.2E+08 & 2.3E+03 & 4.9E+07 & 1.7E+03 & 1.7E+08 & 3.0E-02 & - & - & - & - & - & 3.0E-02 \\
G0.970-0.067 & 11 & 5.9E+07 & 1.7E+03 & 1.4E+07 & 8.8E+02 & 7.3E+07 & 1.3E-02 & - & - & - & - & - & 1.3E-02 \\
G0.840-0.065 & 12 & 5.1E+07 & 2.1E+03 & 1.2E+07 & 8.6E+02 & 6.4E+07 & 1.1E-02 & - & - & - & - & - & 1.1E-02 \\
G0.830-0.062 & 13 & 4.9E+07 & 2.2E+03 & 1.2E+07 & 8.6E+02 & 6.1E+07 & 1.0E-02 & - & - & - & - & - & 1.0E-02 \\
G0.820-0.059 & 14 & 4.0E+07 & 2.3E+03 & 8.5E+06 & 7.9E+02 & 4.9E+07 & 8.4E-03 & - & - & - & - & - & 8.4E-03 \\
G0.800-0.060 & 15 & 3.3E+07 & 2.6E+03 & 6.5E+06 & 7.7E+02 & 4.0E+07 & 6.8E-03 & - & - & - & - & - & 6.8E-03 \\
G359.900-0.071 & 19 & 4.7E+07 & 4.7E+03 & 2.5E+07 & 3.0E+03 & 7.2E+07 & 1.2E-02 & - & - & - & - & - & 1.2E-02 \\
G0.020-0.058 & 27 & 3.6E+07 & 5.2E+03 & 1.9E+07 & 3.6E+03 & 5.4E+07 & 9.3E-03 & - & - & - & - & - & 9.3E-03 \\
G1.610-0.059 & 23 & 3.6E+06 & 5.5E+02 & - & - & 3.6E+06 & 6.2E-04 & - & - & - & - & - & 6.2E-04 \\
G0.670-0.059 & 17 & 2.4E+07 & 3.9E+03 & 4.9E+06 & 8.1E+02 & 2.9E+07 & 4.9E-03 & - & - & - & - & - & 4.9E-03 \\
G0.040-0.054 & 31 & 2.7E+07 & 5.8E+03 & 1.3E+07 & 4.1E+03 & 4.0E+07 & 6.9E-03 & - & - & - & - & - & - \\
G0.650-0.040 & 25 & 1.9E+07 & 4.7E+03 & 3.4E+06 & 8.8E+02 & 2.2E+07 & 3.8E-03 & - & - & - & - & - & - \\
G1.040-0.051 & 29 & 4.8E+06 & 1.4E+03 & 5.9E+05 & 4.8E+02 & 5.4E+06 & 9.4E-04 & - & - & - & - & - & - \\
G359.530-0.120 & 18 & 9.3E+06 & 3.6E+03 & 4.9E+06 & 1.9E+03 & 1.4E+07 & 2.4E-03 & - & - & - & - & - & - \\
G0.670-0.038 & 26 & 1.3E+07 & 5.4E+03 & 2.0E+06 & 8.5E+02 & 1.5E+07 & 2.5E-03 & - & - & - & - & - & - \\
G359.960-0.078 & 32 & 1.3E+07 & 5.8E+03 & 6.9E+06 & 3.9E+03 & 2.0E+07 & 3.4E-03 & - & - & - & - & - & - \\
G0.660-0.023 & 37 & 7.9E+06 & 7.1E+03 & 1.1E+06 & 9.8E+02 & 8.9E+06 & 1.5E-03 & - & - & - & - & - & - \\
G0.210-0.003 & 44 & 5.6E+06 & 5.1E+03 & 2.9E+06 & 4.2E+03 & 8.5E+06 & 1.5E-03 & - & - & - & - & - & - \\
G359.910-0.079 & 34 & 6.8E+06 & 6.3E+03 & 3.1E+06 & 3.6E+03 & 9.9E+06 & 1.7E-03 & - & - & - & - & - & - \\
G0.220-0.490 & 3 & 2.1E+05 & 3.7E+02 & 2.8E+05 & 6.6E+02 & 4.9E+05 & 8.5E-05 & - & - & - & - & - & - \\
G0.110-0.079 & 35 & 1.7E+06 & 4.0E+03 & 1.6E+06 & 4.4E+03 & 3.3E+06 & 5.7E-04 & - & - & - & - & - & - \\
G0.400+0.048 & 50 & 8.5E+05 & 3.3E+03 & 1.9E+05 & 7.6E+02 & 1.0E+06 & 1.8E-04 & - & - & - & - & - & - \\ \hline
Leaves & \\ \hline
G359.510-0.130  & 24 & 4.5E+06 & 3.9E+03 & 2.2E+06 & 1.9E+03 & 6.7E+06 & 1.2E-03 & 7.7E-03 & - 		 & - 		    & -  	     & - 	     & 7.7E-03 \\
G1.070-0.049      & 33 & 1.5E+06 & 1.4E+03 & 3.8E+04 & 4.2E+02 & 1.6E+06 & 2.7E-04 & 4.9E-03 & 7.1E-03  & 4.2E-03   & 1.1E-03  & 6.0E-04 & 7.1E-03 \\
G0.230-0.004      & 45 & 4.1E+06 & 5.1E+03 & 2.7E+06 & 4.2E+03 & 6.8E+06 & 1.2E-03 & 9.5E-03 & -  		 & - 		    & - 	     & - 	     & 9.5E-03 \\
G0.890-0.044      & 39 & 1.3E+06 & 1.8E+03 & 3.4E+05 & 4.7E+02 & 1.6E+06 & 2.8E-04 & 5.4E-03 & -             & -               & -             & -            & 5.4E-03 \\
G0.820-0.190      & 21 & 1.3E+06 & 2.1E+03 & 2.8E+05 & 4.5E+02 & 1.6E+06 & 2.8E-04 & 5.6E-03 & -             & -               & -             & -            & 5.6E-03 \\
G1.720-0.390      & 6   & 1.5E+05 & 2.7E+02 & -             & -              & 1.5E+05 & 2.6E-05 & 1.0E-03 & -             & -               & -             & -            & 1.0E-03 \\
G0.670-0.028      & 43 & 4.9E+06 & 9.6E+03 & 4.7E+05 & 9.5E+02 & 5.4E+06 & 9.2E-04 & 2.6E-02 & -             & -               & -             & -            & 2.6E-02 \\
G0.720-0.090      & 30 & 1.9E+06 & 3.9E+03 & 3.0E+05 & 6.0E+02 & 2.2E+06 & 3.9E-04 & 8.7E-03 & 1.4E-02  & 8.2E-03   & 2.7E-03  & 1.6E-03 & 1.4E-02 \\
G359.690-0.130  & 28 & 1.4E+06 & 2.9E+03 & 7.7E+05 & 1.6E+03 & 2.2E+06 & 3.7E-04 & 4.7E-03 & -             & -               & -             & -            & 4.7E-03 \\
G359.880-0.081  & 36 & 1.9E+06 & 5.1E+03 & 8.5E+05 & 2.4E+03 & 2.8E+06 & 4.8E-04 & 1.2E-02 & 5.1E-02  & 3.0E-02   & 9.2E-03 & 5.5E-03 & 9.2E-03 \\
G1.020-0.230      & 16 & 4.2E+05 & 1.1E+03 & 8.4E+04 & 5.3E+02 & 5.0E+05 & 8.6E-05 & 2.2E-03 & -             & -               & -             & -            & 2.2E-03 \\
G0.550-0.870      & 0   & 6.1E+05 & 1.8E+03 & -             & -             & 6.1E+05 & 1.1E-04 & 2.7E-03 & -              & -               & -             & -            & 2.7E-03 \\
G359.600-0.220  & 20 & 8.6E+05 & 2.7E+03 & 4.8E+05 & 1.5E+03 & 1.3E+06 & 2.3E-04 & 4.6E-03 & -             & -               & -             & -            & 4.6E-03 \\
G0.240-0.470      & 5   & 1.1E+05 & 4.0E+02 & 1.9E+05 & 6.7E+02 & 3.0E+05 & 5.2E-05 & 1.6E-03 & -             & -               & -             & -            & 1.6E-03 \\
G0.490+0.008     & 48 & 1.0E+06 & 4.0E+03 & 1.8E+05 & 7.1E+02 & 1.2E+06 & 2.1E-04 & 8.2E-03 & 1.7E-02  & 1.0E-02   & 2.9E-03  & 1.8E-03 & 1.7E-02 \\
G0.120+0.003     & 46 & 1.2E+06 & 5.0E+03 & -             & -             & 1.2E+06 & 2.1E-04 & 4.7E-03 & 1.7E-03   & 1.0E-03   & 5.0E-04  & 3.0E-04 & 1.7E-03 \\
G1.600+0.012     & 47 & 1.5E+05 & 6.8E+02 & -             & -             & 1.5E+05 & 2.6E-05 & 2.0E-03 & 5.0E-03   & 3.0E-03   & 5.0E-04  & 3.0E-04 & 5.0E-03 \\
G1.650-0.052      & 42 & 1.1E+05 & 5.2E+02 & -             & -             & 1.1E+05 & 1.9E-05 & 1.6E-03 & 1.5E-03   & 9.0E-04   & 2.0E-04  & 1.0E-04 & 1.5E-03 \\
G359.940+0.160 & 54 & 1.7E+05 & 9.2E+02 & 1.6E+05 & 8.2E+02 & 3.3E+05 & 5.7E-05 & 1.9E-03 & -              & -              & -              & -            & 1.9E-03 \\
G0.330-0.190      & 22 & 2.9E+05 & 1.8E+03 & 3.2E+05 & 2.2E+03 & 6.0E+05 & 1.0E-04 & 2.7E-03 & -              & -              & -              & -            & 2.7E-03 \\
G3.430-0.350      & 10 & 5.5E+04 & 3.3E+02 & -             & -             & 5.5E+04 & 9.5E-06 & 6.9E-04 & -               & -              & -              & -            & 6.9E-04 \\
G0.200-0.520      & 4   & 5.4E+04 & 3.4E+02 & 1.5E+04 & 4.7E+02 & 6.9E+04 & 1.2E-05 & 7.9E-04 & -              & -              & -              & -            & 7.9E-04 \\
G0.410+0.048     & 51 & 4.0E+05 & 3.2E+03 & 7.9E+04 & 6.5E+02 & 4.8E+05 & 8.2E-05 & 4.5E-03 & 2.7E-03   & 1.6E-03  & 5.0E-04   & 3.0E-04 & 2.7E-03 \\
G359.980-0.071  & 41 & 9.1E+05 & 8.3E+03 & 4.1E+05 & 5.5E+03 & 1.3E+06 & 2.3E-04 & 9.4E-03 & 6.3E-03   & 3.8E-03  & 1.8E-03   & 1.1E-03 & 6.3E-03 \\
G0.340+0.060     & 53 & 3.5E+05 & 3.5E+03 & 1.2E+05 & 1.2E+03 & 4.7E+05 & 8.1E-05 & 3.5E-03 & -              & -              & -              & -            & 3.5E-03 \\
G0.120-0.081      & 38 & 4.3E+05 & 4.3E+03 & 3.6E+05 & 3.6E+03 & 7.9E+05 & 1.4E-04 & 6.3E-03 & 4.0E-04   & 3.0E-04  & 1.0E-04  &1.0E-04  & 4.0E-04 \\
G358.460-0.390  & 7   & 3.8E+04 & 4.7E+02 & -             & -              & 3.8E+04 & 6.6E-06 & 7.0E-04 & -              & -             & -              & -            & 7.0E-04 \\
G356.660+0.560 & 56 & 1.8E+03 & 3.0E+01 & -             & -              & 1.8E+03 & 3.2E-07 & 2.0E-04 & -              & -             & -              & -            & 2.0E-04 \\
G0.070-0.076      & 40 & 2.2E+05 & 3.8E+03 & 2.9E+05 & 6.4E+03 & 5.1E+05 & 8.8E-05 & 6.1E-03 & 6.4E-03   & 3.8E-03  & 1.5E-03  & 9.0E-04 & 6.4E-03 \\
G0.090-0.660      & 2   & 2.8E+04 & 5.3E+02 & -             & -              & 2.8E+04 & 4.8E-06 & 6.1E-04 & -              & -             & -              & -            & 6.1E-04 \\
G0.380+0.050     & 52 & 1.7E+05 & 3.7E+03 & 3.7E+04 & 8.0E+02 & 2.1E+05 & 3.6E-05 & 3.3E-03 & 3.9E-02   & 2.3E-02  &  1.0E-02 & 6.1E-03 & 1.0E-02 \\
G356.520+0.210 & 55 & 1.8E+03 & 4.7E+01 & -             & -              & 1.8E+03 & 3.2E-07 & 2.3E-04 & -              & -             & -              & -            & 2.3E-04 \\
G357.070-0.770  & 1   & 3.5E+02 & 1.3E+01 & -             & -              & 3.5E+02 & 6.0E-08 & -            & -              & -             & -              & -            & 6.0E-08 \\
G0.650+0.030     & 49 & 1.1E+05 & 3.8E+03 & 1.2E+04 & 3.9E+02 & 1.3E+05 & 2.2E-05 & 4.1E-03 & -              & -             & -              & -            & 4.1E-03 \\ \hline \hline

\end{tabular}%
\label{tab:luminosity_properties}
}
\end{table*}

